Context-dependent Instruction Tuning for Dialogue Response Generation

Recent language models have achieved impressive performance in natural language tasks by incorporating instructions with task input during fine-tuning. Since all samples in the same natural language task can be explained with the same task instructions, many instruction datasets only provide a few instructions for the entire task, without considering the input of each example in the task. However, this approach becomes ineffective in complex multi-turn dialogue generation tasks, where the input varies highly with each turn as the dialogue context changes, so that simple task instructions cannot improve the generation performance. To address this limitation, we introduce a context-based instruction fine-tuning framework for each multi-turn dialogue which generates both responses and instructions based on the previous context as input. During the evaluation, the model generates instructions based on the previous context to self-guide the response. The proposed framework produces comparable or even outstanding results compared to the baselines by aligning instructions to the input during fine-tuning with the instructions in quantitative evaluations on dialogue benchmark datasets with reduced computation budget.

==> Table/old_1_main_table.tex <==
\begin{table*}[t]\centering
\centering
\begin{adjustbox}{width=\textwidth}
% PPL BLEU NIST-4 BSf Ent-1 Ent-2 Ent-3 Dis-1 Dis-2 Dis-3 C
\begin{tabular}{lcccccccccc}
\toprule
 \multicolumn{1}{l|}{\textbf{Model}} &
 \multicolumn{1}{c}{BLEU} & 
 \multicolumn{1}{c}{NIST-4} & 
 \multicolumn{1}{c|}{{$\text{BS}_{f}$}} &
 \multicolumn{1}{c}{Ent-1} & 
 \multicolumn{1}{c}{Ent-2} & 
 \multicolumn{1}{c}{Ent-3} & 
 \multicolumn{1}{c}{Dis-1} & 
 \multicolumn{1}{c}{Dis-2} & 
 \multicolumn{1}{c|}{Dis-3} & 
 \textbf{C-score}\\
\midrule[0.5pt]
 \multicolumn{1}{l|}{Transformer} &
 \multicolumn{1}{c}{3.140} & 
 \multicolumn{1}{c}{1.148} & 
 \multicolumn{1}{c|}{0.1486} &
 \multicolumn{1}{c}{4.076} & 
 \multicolumn{1}{c}{5.484} & 
 \multicolumn{1}{c}{6.262} & 
 \multicolumn{1}{c}{1.609} & 
 \multicolumn{1}{c}{6.298} & 
 \multicolumn{1}{c|}{11.71} & 
 0.235 \\ % result from D3 
 \multicolumn{1}{l|}{GPT2} &
 \multicolumn{1}{c}{3.761} & 
 \multicolumn{1}{c}{1.278} & 
 \multicolumn{1}{c|}{0.1693} &
 \multicolumn{1}{c}{4.485} & 
 \multicolumn{1}{c}{6.187} & 
 \multicolumn{1}{c}{7.029} & 
 \multicolumn{1}{c}{2.011} & 
 \multicolumn{1}{c}{8.260} & 
 \multicolumn{1}{c|}{15.03} & 
 0.518 \\ % result from D3 
 \multicolumn{1}{l|}{BoB} &
 \multicolumn{1}{c}{2.504} & 
 \multicolumn{1}{c}{1.429} & 
 \multicolumn{1}{c|}{0.1910} &
 \multicolumn{1}{c}{4.956} & 
 \multicolumn{1}{c}{6.877} & 
 \multicolumn{1}{c}{8.176} & 
 \multicolumn{1}{c}{3.451} & 
 \multicolumn{1}{c}{13.23} & 
 \multicolumn{1}{c|}{26.49} & 
 0.088 \\
 \multicolumn{1}{l|}{$\text{GPT2-D}^3$} &
 \multicolumn{1}{c}{4.184} & 
 \multicolumn{1}{c}{1.429} & 
 \multicolumn{1}{c|}{0.1835} &
 \multicolumn{1}{c}{4.614} & 
 \multicolumn{1}{c}{6.426} & 
 \multicolumn{1}{c}{7.321} & 
 \multicolumn{1}{c}{2.267} & 
 \multicolumn{1}{c}{9.803} & 
 \multicolumn{1}{c|}{18.20} & 
 0.557\\

\midrule[0.5pt]
 %small
 \multicolumn{1}{l|}{Original Flan-T5} &
 \multicolumn{1}{c}{5.189} & 
 \multicolumn{1}{c}{1.871} & 
 \multicolumn{1}{c|}{0.2198} &
 \multicolumn{1}{c}{5.074} & 
 \multicolumn{1}{c}{6.743} & 
 \multicolumn{1}{c}{7.867} & 
 \multicolumn{1}{c}{3.999} & 
 \multicolumn{1}{c}{12.83} & 
 \multicolumn{1}{c|}{23.30} & 
 0.781\\
 \multicolumn{1}{l|}{InstructDial Flan-T5} &
 \multicolumn{1}{c}{4.591} & 
 \multicolumn{1}{c}{1.606} & 
 \multicolumn{1}{c|}{0.2070} &
 \multicolumn{1}{c}{5.087} & 
 \multicolumn{1}{c}{6.782} & 
 \multicolumn{1}{c}{7.922} & 
 \multicolumn{1}{c}{3.749} & 
 \multicolumn{1}{c}{11.53} & 
 \multicolumn{1}{c|}{21.25} & 
 1.000\\
\midrule[0.5pt]
 \multicolumn{1}{l|}{Our Flan-T5} &
 \multicolumn{1}{c}{6.776} & 
 \multicolumn{1}{c}{2.216} & 
 \multicolumn{1}{c|}{0.2602} &
 \multicolumn{1}{c}{5.073} & 
 \multicolumn{1}{c}{6.719} & 
 \multicolumn{1}{c}{7.818} & 
 \multicolumn{1}{c}{4.569} & 
 \multicolumn{1}{c}{14.27} & 
 \multicolumn{1}{c|}{25.42} & 
 0.647\\
\midrule[0.5pt]
 \multicolumn{1}{l|}{Human} &
 \multicolumn{1}{c}{-} & 
 \multicolumn{1}{c}{-} & 
 \multicolumn{1}{c|}{-} &
 \multicolumn{1}{c}{5.704} & 
 \multicolumn{1}{c}{8.943} & 
 \multicolumn{1}{c}{10.27} & 
 \multicolumn{1}{c}{5.464} & 
 \multicolumn{1}{c}{36.69} & 
 \multicolumn{1}{c|}{67.82} & 
 0.472\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\label{convai2_table} \textbf{Performance of ConvAI2 dataset.} We compared the response quality and diversity of three baselines.} 
\end{table*}


==> Text/5_analyses.tex <==
\section{Analysis}

==> Text/8_acknowledge.tex <==
\section*{Acknowledgements}


